SEAL: Segment-wise Extractive-Abstractive Long-form Text Summarization

Most prior work in the sequence-to-sequence paradigm focused on datasets with input sequence lengths in the hundreds of tokens due to the computational constraints of common RNN and Transformer architectures. In this paper, we study long-form abstractive text summarization, a sequence-to-sequence setting with input sequence lengths up to 100,000 tokens and output sequence lengths up to 768 tokens. We propose SEAL, a Transformer-based model, featuring a new encoder-decoder attention that dynamically extracts/selects input snippets to sparsely attend to for each output segment. Using only the original documents and summaries, we derive proxy labels that provide weak supervision for extractive layers simultaneously with regular supervision from abstractive summaries. The SEAL model achieves state-of-the-art results on existing long-form summarization tasks, and outperforms strong baseline models on a new dataset/task we introduce, Search2Wiki, with much longer input text. Since content selection is explicit in the SEAL model, a desirable side effect is that the selection can be inspected for enhanced interpretability.

==> figs/wikifull.tex <==
\definecolor{c1}{rgb}{0.9, 0.17, 0.31}
\definecolor{c2}{rgb}{0.36, 0.54, 0.66}
\definecolor{c3}{rgb}{0.55, 0.71, 0.0}
\definecolor{c4}{rgb}{0.8, 0.5, 0.2}


\begin{figure}
\fbox{
\centering
\begin{minipage}{18em}
\small

\textbf{Decode} \\
\textcolor{c1}{CLC (Hangul: 씨레씨; short for "CrystaL Clear") is a seven-member South Korean girl group formed by Cube Entertainment in 2015. The group consists of Seunghee, Yujin, Seungyeon, and}\textcolor{c2}{yeon. The group was later renamed CLC and was officially named ambassador to the Korea Insulin Dependent Diabetes Association in November 2015.
The group debuted on March 5, 2015 with First Love, issuing a blitz of EPs into the end of the decade that kept them planted}\textcolor{c3}{in the Korean Top 20 until their 2017 U.S. breakthrough, Crystyle, expanded their international audience. In 2019 they hit a chart peak in Korea and the U.S. with their eighth Korean-language effort, No. 1. Following their eighth Korean-language effort, Crystyle, which included}\textcolor{c4}{the HyunA-assisted EDM trap banger, "Hobgoblin", CLC released their first digital single, "To the Sky", on February 1, 2017, followed by the seventh extended play, Black Dress, on February 22. CLC held their third anniversary Black}\textcolor{c5}{s concert on April 1, which was a donation-based charity show, with proceeds going to the Diabetes Association. Later that year, CLC was officially named as the ambassador to the Korea Insulin Dependent Diabetes Association in November.
On February 12, 2018, CLC released}\textcolor{c6}{their first digital single, "To the Sky", which was released on February 1, followed by the seventh extended play, Black Dress. On February 22, CLC held their third anniversary Black Dress concert, which was a donation-based charity show, with proceeds going to the Diabetes Association. }\textcolor{c7}{Later that year, CLC was officially named as the ambassador to the Korea Insulin Dependent Diabetes Association in November.

== Singles ==

"No" (February 12, 2019)
"No}\textcolor{c8}{ (March 2, 2019)
"Hobgoblin" (February 22, 2019)
"Hobgoblin" (February 1, 2019)
"Hobgoblin" (February 1, 2019)
"No}\textcolor{c9}{
}
\\ \textbf{Input} \\
... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... This means that the team will not get any presale tokens. 
 \textcolor{c1}{(1)}\textcolor{c1}{Related reads Related reads Related reads CLC Group CLC Group is a blockchain lab focused on developing real-world connected smart contract solutions... 
} Home - clc group of nj - custom builders serving ocean/monmouth LIVE 0 00:00 00:00 Click to Unmute Player error The player is having trouble. 
 ... ... ... read more Port Equipment Manufacturers Association welcomes four new Members ZPMC, Nantong Heavy Rainbow Machineries, Spohn + Burkhardt and INTERCON Technical Information System... 
 \textcolor{c1}{(1)}\textcolor{c1}{read more University of hamburg team win PEMA Student challenge for second year running June 29, 2018 -- The Port Equipment Manufacturers Association (PEMA) hosts the PEMA Student Ch... 
} http://clc-enterprises.com/ < previous page Contacts Login OUR MEMBERS Samson Materials Handling Ltd. 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... Earthquake Assessments Fire Reports Resource Management - Resource consents and town planning Land Surveying - Topographical and boundaries. 
 \textcolor{c1}{(1)}\textcolor{c1}{Clc group ZoomInfo.com Platform Clc group Location: Taiwan Revenue: \$3 Million Employees: 15 Website: www.clc-enterprises.com Description: CLC Group is a company group founded in 1978 in Taiwan. 
} Philip Charles Procurement Officer Wilson Wong Vice General Manager 2 Contacts fromCLC Group 2 Contacts from CLC Group Browse Our Directories
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... CLC become the girl group that took the longest time in getting their first music show win Allkpop 99 16 News Posted by yckim124 Tuesday, February 12, 2019 CLC become the girl group that took the longest time in getting their first music show win AKP STAFF CLC made a new record with their first win. 
 \textcolor{c7}{(7)}\textcolor{c7}{On the February 12 airing of SBS FunE's 'The Show,' CLC with their new song ``No'' finally achieved their very first music show win. 
} Previously, the title was held by Girl's Day who took their first trophy home after 1,098 days since their debut. 
 ... ... ... ... 3 Jun 2019 Magazines Get make-up tips from these 9 Muslim beauty influencers 13 Jun 2019 Magazines K-pop star Jessica Jung's 5 most fashionable moments 24 May 2019 Magazines 6 things to know about K-pop acts for SBS Super Concert 11 Jun 2019 Magazines 4 things you didn't know about K-pop star Tzuyu of TWICE 14 Jun 2019 CLC performs Show at the unveiling of its eighth mini album '
 \textcolor{c8}{(8)}\textcolor{c8}{Photo: Courtesy of Cube Entertainment K-pop girl group CLC released its eighth mini album ``No.1'' on Wednesday, fronted by the single No as it revealed a chic, elegant concept full of glam looks. 
} During the group's hiatus, the members have been busy in a number of individual activities, appearing on reality shows, drama series and with Elkie launching a solo career. 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... CLC debut on World Digital Song sales & World Albums charts thanks to 'Hobgoblin' CLC also make their first appearance on the Heatseekers Albums chart with No.1 starting at No. 
 \textcolor{c8}{(8)}\textcolor{c8}{Previous to No.1, CLC had landed three entries only World Albums. 
} \textcolor{c8}{(8)}\textcolor{c8}{Notably, all of CLC's albums to enter the Top 10 or higher on World Albums have all seen the group showcasing a fiercer side of their image. 
} A quick switch back to a retro-influenced innocence with the citypop-inspried single ``Where Are You'' off their Free'sm knocked them down to No. 
 \textcolor{c8}{(8)}\textcolor{c8}{1thek (원더케이) 16m subscribers (MV) CLC _ No Share Share 0:00 / 3:04 Live Elsewhere on Billboard's World Digital Song Sales chart, CLC's new single ``No'' debuts at No. 
} ``No'' ties CLC's previous best on the chart when 2017's ``Hobgoblin'' also hit No. 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... Six months later, that dream came true. 
 \textcolor{c7}{(7)}\textcolor{c7}{With their hard work and support from ARMYs, BTS became global superstars. 
} \textcolor{c7}{(7)}\textcolor{c7}{The seven-member group released their eighth mini-album ``No. 
} \textcolor{c8}{(8)}\textcolor{c8}{The K-pop : sbs plus 376k subscribers CLC's THE FIRST WIN! 
} They performed ``Dramarama,'' the lead single from their album ``The Code,'' on ``The Show'' on November 14, 2017. 
 \textcolor{c8}{(8)}\textcolor{c8}{GOT7 - ``If You Do'' (October 6, 2015) Boy band GOT7 got their first taste of music show win on October 6, 2015 on ``The Show.'' GOT7 debuted in January 2014 and in September 2015, they released the album ``MAD,'' containing the title track ``If You Do.'' The song, with a score of 8,981, won them their first-ever TV music program trophy on ``The Show'' as they competed for the Choice with CNBLUE, 
} Bambam kissdatbam 11k subscribers (ENGSUB) 151006 GOT7 1st Win @ The Show Switch camera 0:00 0:00 0:00 / 2:38 Live ASTRO - ``All Night'' (January 29, 2019) Boy band ASTRO made their comeback last January with the album ``All Night'' after 14 months' break. 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... Jenna Lemoncelli Entertainment & Sports Editor CLC finally released their heavily teased music video for 'no' on January 30, and we can't stop watching! 
 \textcolor{c8}{(8)}\textcolor{c8}{-- CLC has the internet buzzing over the music video for their smash hit ``No''! 
} But, they all come together with their matching red lips, dangling earrings and sky high heels. 
 ... ... ... I FELT THAT.@CUBECLC #CLC #No #No_1 #씨엘씨 #Comeback #CLC_NO_1 pic.twitter.com/Fawn2d9DUu -- Yellow Banana~��ia (@Clo_BnanaInjeol) January 30, 2019 MISS SEUNGYEON CAME FOR BLOOD #CLC_No_1 pic.twitter.com/
 \textcolor{c8}{(8)}\textcolor{c8}{The group had a busy year in 2018, having released their digital single, ``To The Sky'' on February 1, followed by the seventh extended play, Black Dress, on February 22. 
} The White Buffalo Will Move You With His Music More Videos Next Up The Who: Moving On! 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... It was released on January 30, 2019, with ``No'' serving as the album's title track. 
 \textcolor{c8}{(8)}\textcolor{c8}{``No'' music video M/V teaser Behind the scenes: Part 1 / 2 Members teasers: Seunghee / Yujin / Seungyeon / Sorn / Yeeun / Elkie / Eunbin ``No'' selfie music video ``No'' dance practice Silhouette ver. 
} ``Like It'' dance practice ``No'' relay dance video ``No'' fan greeting guide video Comeback showcase ``No'' performance Teaser Album preview Album photoshoot making-of: Part 1 / 2 CLC Seungyeon Yujin Seunghee Sorn Yeeun Elkie Eunbin Discography Korean Mini albums First Love Question Refresh Nu.Clear Crystyle Free'sm Black Dress No.1 Digital singles ``Eighteen'' ``To the Sky'' ``Me
 ... ... ... ... ... ... ‎CLCon Apple music Global Nav Open Menu Global Nav Close Menu Apple Shopping Bag Search apple.com Cancel Apple Mac iPad iPhone Watch TV Music Support Shopping Bag Cancel Apple Music Preview Sign Out Sign In Try It Now Get Apple Music on iOS, Android, Mac, and Windows Learn More CLC View on Apple Music Latest Release May 30, 2019 ME - Single 1 song Top Songs See All ME ME - Single
 \textcolor{c7}{(7)}\textcolor{c7}{The first all-girl outfit for Cube Entertainment, the seven-piece CLC debuted in early 2015 with First Love, issuing a blitz of EPs into the end of the decade that kept them planted in the Korean Top 20 until their 2017 U.S. 
} \textcolor{c2}{(2)}\textcolor{c2}{Originally a quintet that served a stint as backup for Canadian-born Korean singer G.NA, CLC's first incarnation consisted of leader Seungyeon, Seunghee, Yujin, Yeeun, and Thai member Sorn. 
} Coinciding with the fresh additions, they issued their first offering as a septet, the aptly titled Refresh. 
 \textcolor{c5}{(5)}\textcolor{c5}{Shifting in an edgier direction in 2017, they released Crystyle, which included the HyunA-assisted EDM trap banger, ``Hobgoblin.'' While the EP marked their first placement on the U.S. 
} That summer, Free'sm arrived, an R&B/pop throwback to iconic predecessors like Fin.K.L and S.E.S. 
 ... ... ... ... ... ... ... ... ... ... It's a safe place to share. 
 \textcolor{c1}{(1)}\textcolor{c1}{Kate Waggoner clc network KpopClc HobgoblinTumblr WallpaperKorean Girl Groups love and support these girls~ ♡ Kate Waggoner CLC Clc HobgoblinCheshireKpop FashionKorean FashionKorean GroupKpop GirlsFandomsCrystalsGirl Group This is a network dedicated to the seven-member girl group Crystal Clear! 
} \textcolor{c1}{(1)}\textcolor{c1}{Kate Waggoner South Korean GirlsKorean Girl GroupsCube EntertainmentClcKpop GroupsDistanceGirls Girls GirlsApril 3News CLC revela MV para ``Distance'' Kate Waggoner CLC CLC network Pretty Korean GirlsSouth Korean GirlsK PopCube EntertainmentClcUlzzangKorean Girl GroupsFandomKpop Groups This is a network dedicated to the seven-member girl group Crystal Clear! 
} It's a safe place to share our love for these amazing hardworking girls so if you love CLC. 
 ... ... ... ... ... Kate Waggoner Kpop Girl GroupsKpop GirlsCube EntClcMamamooNayeonBias WreckerRed VelvetGot7 Kate Waggoner BaekhyunKpop Girl GroupsKorean Girl GroupsKpop GirlsK PopKpop OutfitsStage OutfitsClc HobgoblinCube Entertainment Read 041 from the story Se Você Fosse Um K-idol by sillyukhei (☁ 
 \textcolor{c1}{(1)}\textcolor{c1}{Abby Lynn K-pop ruined me CLC (씨엘씨/ 處理廠) CLC network Clc HobgoblinK IdolKorean Girl GroupsKpop Girl GroupsKpop GirlsGot7Korean FashionKpop FashionFandom This is a network dedicated to the seven-member girl group Crystal Clear! 
} Amanda Leal Idol International Playboy Girl groups Clc HobgoblinK PopKpop Girl GroupsKorean Girl GroupsKpop GirlsCube EntertainmentTwiceIkonUlzzang This is a network dedicated to the seven-member girl group Crystal Clear! 
 ... ... ... ... ... Travel ⚓ Love Girls Black DressGroup PhotosKpop GirlsKpop Girl GroupsKorean Girl GroupsEuna KimJang YeeunCubesK Pop *CLC (씨엘씨) currently consists of 7 members. 
 \textcolor{c2}{(2)}\textcolor{c2}{The band debuted on March under Cube Entertainment Anita༺♥༻ Anita༺♥༻ ✨K-Pop is My Inspiration ✨✨ ♫ ♫ IdoleKpop FashionKorean FashionKpop Girl GroupsKorean Girl GroupsKpop GirlsStage OutfitsKpop OutfitsFandom 170208 CLC (씨엘씨) Elkie (엘키) Skye Dickerson
} Queen Stacie CLC - Eunbin #kpop South Korean GirlsKorean Girl GroupsKpop Girl GroupsKpop GirlsCheshireClcSamsungCube EntertainmentGirl Bands Kath CheshireKpop Girl GroupsKpop GirlsClcKorean OutfitsUlzzangBabysAppreciationGoddesses I like it sorn and yujin Kate Waggoner ClcKpop GirlsFandomCheshireCube
 ... ... ... ... ... Clc music, videos, stats, and photos Last.fm More... 
 \textcolor{c2}{(2)}\textcolor{c2}{Similar Artists Events Listeners 2.9M 51.2K Six-month listening trend Created with Highcharts 5.0.6 Play on youtube ME 4,974 listeners Play album ME 1 track k-pop girl group korean kpop pop dance Seoul, Korea, Republic of (2015 -- present) CLC (씨엘씨; short for ``CrystaL Clear'') is a seven-member South Korean girl group formed by Cube Entertainment in 2015. 
} \textcolor{c4}{(4)}\textcolor{c4}{The group consists of Seunghee, Yujin, Seungyeon... 
} read more Last 7 days 1 Play on youtube ME 4,974 listeners 2 Play on youtube No 4,112 listeners 3 Play on youtube BLACK DRESS 2,440 listeners 4 Play on youtube Hobgoblin 1,964 listeners 5 Play on youtube Like It 1,280 listeners 6 Play on youtube SHOW 904 listeners 7 Play on youtube I Need U 862 listeners 8 Play on youtube I LIKE IT 652 listeners 9 Play on youtube Liar 607 listeners 10 Play on youtube
 ... ... ... ... ... ... ... ... ... Actions 24 23 More shouts clcno yemoum Jiwoo_biased Audreyoongii Charts & Trends Last.fm's Hype Chart (Week 23 of 2019) Charts & Trends Last.fm's Hype Chart (Week 22 of 2019) Spotlight 35 years later, Mariya Takeuchi's 'Plastic Love' has an official music video Charts & Trends Last.fm's Hype Chart (
 \textcolor{c3}{(3)}\textcolor{c3}{CLC worship band CLC Worship BandKeith2018-01-29T16:49:10-07:00 The CLC worship band leads the congregation at the 11:15 a.m. 
} The music varies from hymns played in the contemporary style for a band, songs by new artists, and traditional praise songs. 
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... CLC ME 3:130:30 No 3:010:30 BLACK DRESS 3:130:30 Hobgoblin 3:300:30 Like It 3:130:30 Korean girl group CLC bring attitude and edge to their beat-forward K-pop anthems, which lean more on fun dance energy than sweet balladry. 
 \textcolor{c7}{(7)}\textcolor{c7}{The second all-girl outfit for CUBE Entertainment, the seven-piece CLC debuted in early 2015 with First Love, issuing a blitz of EPs into the end of the decade that kept them planted in the Korean Top 20 until their 2017 U.S. 
} \textcolor{c8}{(8)}\textcolor{c8}{CLC's incarnation consisted of leader OH SEUNGHEE, CHOI YUJIN, CHANG SEUNGYEON, SORN, JANG YEEUN, ELKIE and KWON EUNBIN. 
} Months later, they released their first Japanese-language effort, High Heels, which included a cover of Kylie Minogue's 1987 hit ``I Should Be So Lucky.'' Back in the Korean market, they released Nu.Clear that May and their second Japanese EP Chamisma in July. 
 \textcolor{c4}{(4)}\textcolor{c4}{Continuing their musical maturation, the ``No''-featuring set peaked in the Top Five in both Korea and on the U.S. 
} Yeung, Rovi Read More 360,857 Jakarta, ID35,670 LISTENERS Singapore, SG29,776 LISTENERS Bangkok, TH23,799 LISTENERS Santiago, CL17,124 LISTENERS Kuala Lumpur, MY16,701 LISTENERS ME No.1 BLACK DRESS To the sky FREE`SM CRYSTYLE チャミスマNU.CLEAR K-Pop
 Listen to CLC in full in the Spotify app Playing CLC Playing CLC
 \textcolor{c1}{(1)}\textcolor{c1}{Clc Discography & songs Discogs Box Set 284,416 Clc (2) Profile: CLC (Hangul: 씨엘씨) is a seven-member South Korean girl group formed by Cube Entertainment in 2015. 
} Sites: Facebook, YouTube, Twitter, instagram.com Members: Kwon Eun Bean, Seung Hee, Seung Yeon, Sorn, Ye Eun, Yu Jin (3) (a4448626) 9 Releases 8 Albums 1 Singles & EPs 1 Recent Releases 9 submissions pending 1 -- 9 of 9 Albums CMCC10576 CLC (2) Question (CLC 2nd Mini Album) ‎(CD, MiniAlbum) Cube Entertainment
 ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... ... CLC get their first ever win on a music program on 'the Show' Kpopmap #SOMI #Debut #Showcase #MakeYouFallinLove #Upcoming #June #Latest #Kpop #MV #PRODUCEX101 #ShouldKnow Challenge to Become a True ``CHERRY BULLET'' Fan #SOMI #Debut #Showcase #MakeYouFallinLove #Upcoming #June #Latest #Kpop #
 \textcolor{c7}{(7)}\textcolor{c7}{The statement rings true to K-Pop idol girl group CLC even more so at the moment as they recently had their first ever win on a music program. 
} After debuting in 2015, their recent accomplishment has been a milestone in their career since despite having a substantial fan base in the overseas K-Pop market, they were unable to have the same prominence in the domestic market in South Korea. 


 
 
 \end{minipage}
}
\caption{Visualization of the SEAL model on an CNN/DailyMail example. Segments of decodes are colored differently. Input snippets each segment attends to are are colored accordingly and the segment ids are inserted to the front. When multiple segment attend to the same input snippet, it is colored as the first segment.}
\label{fig:interp}

\end{figure}

